Autoregressive Knowledge Distillation through Imitation Learning

The performance of autoregressive models on natural language generation tasks has dramatically improved due to the adoption of deep, self-attentive architectures. However, these gains have come at the cost of hindering inference speed, making state-of-the-art models cumbersome to deploy in real-world, time-sensitive settings. We develop a compression technique for autoregressive models that is driven by an imitation learning perspective on knowledge distillation. The algorithm is designed to address the exposure bias problem. On prototypical language generation tasks such as translation and summarization, our method consistently outperforms other distillation algorithms, such as sequence-level knowledge distillation. Student models trained with our method attain 1.4 to 4.8 BLEU/ROUGE points higher than those trained from scratch, while increasing inference speed by up to 14 times in comparison to the teacher model.

==> formulation.v1.tex <==
%\section{Connecting Autoregressive Distillation with Imitation Learning}
\section{Problem Formulation}
%\hc{High level comment on style: we can be more direct in terms of laying out the method and provide "reasoning" in a more compact fashion.}
We introduce notations and formalize the task of autoregressive distillation in this section.
Consider an \emph{autoregressive model} $\pi$ which specifies a distribution over a $T$-dimensional \emph{target variable} $\bd y = \{y_1, \ldots, y_T\} \in \mathcal{Y}$ by decomposing its joint distribution into a product of univariate conditionals:
\begin{align}
\pi(\bd y) = \prod_{t=1}^T  \pi(y_t \given \bd y_{<t}),
\end{align}
where $\bd y_{<t}$ denotes $\{y_1, \ldots, y_{t-1}\}$ for $t > 1$ and $\emptyset$ for $t = 1$.  The joint distribution over $\bd y$ may itself be conditional on some related \emph{source feature} $\bd x \in \mathcal{X}$ (e.g. translation, summarization) or not (e.g. language modeling).  %For notational simplicity, we will omit the presence of $\bd x$ for the remainder of the manuscript.
Since the former case can generalize the latter by letting $\mathcal{X} = \emptyset$, we will specify the presence of $\bd x$ in the remainder of the manuscript. 

In autoregressive distillation, the goal is to learn a \emph{student model} $\pi$ by minimizing its loss with respect to a pre-trained \emph{teacher model} $\pi^*$.
In many cases, the training objective can be formalized as:
\begin{align*}
\Loss(\pi) &=\, \E_{\,\bd y | \bd x \sim \mathcal{D}} \left[\ \ell_\pi^{\pi^*}(\bd y | \bd x) \ \right] \\
&=\, \E_{\,\bd y | \bd x \sim \mathcal{D}} \left[\sum_{t} \ell_\pi^{\pi^*}(y_t | \bd y_{<t}, \bd x) \right]
\end{align*}
where $\mathcal{D}$ denotes a distribution (or a dataset) consisting of example generations $\bd x \rightarrow \bd y$,
and $\ell_{\pi}^{\pi^*}()$ is the loss function comparing the discrepancy between the teacher and student models (in terms of the conditional distribution $\bd y| \bd x$).

Due to the combinatorial nature of sequence generation, a distillation method must maximize its learning efficiency by (1) carefully selecting the distribution $\mathcal{D}$, i.e. how it explores the combinatorial space, and (2) defining a proper loss function $\ell_\pi^{\pi^*}$ to best leverage supervision signal.
To this end, we motivate our method from the field of \emph{imilation learning}, an active research area of reinforcement learning.

\subsection{Distillation as Imitation Learning}

The dominant methodology for training an autoregressive model is to minimize the negative log-likelihood (NLL) of the observed data $\bd y' \given \bd x' \sim \mathcal{D}'$ over a dataset $\mathcal{D}'$:
\begin{align}
&\Loss_{\text{NLL}}(\pi) = \E_{\bd y'| \bd x' \sim \mathcal{D}'} \left[-\log \pi(\bd y' \given \bd x')\right] \label{nll} \\
&= \E_{\bd y'| \bd x' \sim \mathcal{D}'} \left[- \sum_{t=1}^T \log \pi({y}'_t \given \bd y'_{<t}, \bd x') \right]. \nonumber
\end{align}
This training objective is also called \emph{teacher forcing}, because the true context $\bd y'_{<t} \given \bd x'$ from the data is provided to the model at every time step $t$.

% At test time, the true target $\bd y'$ is unavailable, so the model must tackle the problem of \emph{generation} -- i.e. producing a $T$-step prediction $\bhat{y}$ from scratch given $\bd x'$.  Autoregressive models do this by repeatedly generating a new token $\hat{y}_t$ given its own previously generated context $\bhat{y}_{<t}$ for all $t$.   


% \subsection{Knowledge Distillation}

% Given observed data $\mathcal{D}'$ with input $\bd x' \in \mathcal{X}$ and output ${y}' \in \mathcal{Y}$, the KD training objective minimizes the cross entropy between the output distributions of the teacher model $\pi^*$ and the student model $\pi$,
% \begin{align}
% &\E_{\bd x' \sim \mathcal{D}'} \left[-\sum_{y \in \mathcal{Y}} \pi^*(y \given \bd x') \log \pi(y \given \bd x')\right]. \label{kd}
% \end{align}  
% Equation \ref{kd} shows that the standard KD training objective allows the student model to leverage the teacher's distributional information over \emph{all} elements of $\mathcal{Y}$.  Several works \citep[e.g.][]{tang2019distilling} have empirically demonstrated that this training signal is superior to the original labeled output $y'$.

\subsection{Autoregressive Knowledge Distillation}

% Standard KD is effective in settings such as text classification, in which the output $y$ is one of a few discrete classes.  However, in natural language generation problems, Equation \ref{kd} quickly becomes intractable; the output $\bd y \in \mathcal{Y}$ is a sequence of words $y_1, y_2, \ldots, y_T$ where each $y_t \in \mathcal{V}$ and the output space grows exponentially (i.e. $|\mathcal{Y}| = |\mathcal{V}|^T$).

The seqKD algorithm \citep{kim2016sequence} tackles the problem of how to train a student autoregressive model $\pi$ using a pretrained teacher $\pi^*$.  Given each $\bd y' \given \bd x' \in \mathcal{D}'$, seqKD simply replaces the original $\bd y'$ with the teacher's (approximate) mode $\bd y^* = \arg \max_{\bd y} \pi^*(\bd y \given \bd x')$, which is typically found using beam search.  This forms a teacher-modified dataset $\mathcal{D}^*$, which the student uses for standard NLL training (Equation \ref{nll}):
\begin{align}
\Loss_{\text{seqKD}}(\pi) &= \E_{\bd y^*|\bd x' \sim \mathcal{D}^*} \left[- \log \pi(\bd y^*|\bd x')\right]. \label{seqkd}
\end{align}
Thus, seqKD is teacher forcing with $\mathcal{D}^*$.  Its attractiveness lies in the fact that the method introduces no additional training overhead other than the cost to create the teacher-modified dataset.  

Although this simplicity of seqKD is a nice feature, we conjecture that there are improvements that can be made.  The teacher is a dynamic, query-able entity capable of interacting with the student and can do more than produce a static dataset.  

% There are two established solutions to deal with this issue.  The first is \emph{word-level knowledge distillation} (wordKD), which applies Equation \ref{kd} at the token level of the output.  This yields the following objective:
% \begin{align}
% &\min_\theta \Loss_{\text{wordKD}}(\theta) \label{wordKD} \\
% &= -\frac{1}{T} \sum_{t=1}^T \entr[\pi^*(Y_t \given \bd y_{<t}, \bd x) \dgiven \pi_\theta(Y_t \given \bd y_{<t}, \bd x)] \nonumber \\
% &= -\frac{1}{T} \sum_{t=1}^T \sum_{y_t' \in \mathcal{V}} \pi^*(y_t' \given \bd y_{<t}, \bd x) \log  \pi_\theta(y_t' \given \bd y_{<t}, \bd x), \nonumber
% \end{align}
% where $\bd y_{<t} = \{y_1, \ldots, y_{t-1}\}$ is the true context at time $t$ from the original data.  


% \section{Autoregressive Distillation \& Imitation Learning} 

% We draw connections between knowledge distillation for autoregressive models and the field of imitation learning (IL).  In particular, the teacher-student framework of KD forms a nice parallel with the expert-learner framework of IL.  We show that any teacher forcing training method with a static dataset (such as seqKD) can be interpreted as an IL method known as behavioral cloning, which has known pathologies in the IL community.  This analogy gives us some insight into how we can develop an alternate distillation algorithm.   

\subsection{Generation as an RL Problem} \label{generation-RL}
\hc{To later leverage teacher as a query-able oracle, we draw the connection between autoregressive generation and reinforcement learning.}
At test time, the true target $\bd y'$ is unavailable, so the autoregressive model $\pi$ must tackle the problem of \emph{generation} -- i.e. producing a $T$-step prediction $\bhat{y}$ from scratch given $\bd x'$.  The model does this by repeatedly generating a new token $\hat{y}_t$ given its own previously generated context $\bhat{y}_{<t}$ for all $t$.        

This generation procedure can be interpreted as a Markov decision process (MDP), where the policy we wish to learn is the autoregressive model $\pi$.  The policy $\pi$ maps states $s \in \mathcal{S}$ to distributions over actions $a \in \mathcal{A}$.  Here, $\mathcal{S}$ is the set of all possible contexts (i.e. partial sequences) $\bd y_{<t}$ for any $t < T$ and $\mathcal{A}$ is the set of all possible options for the next token $y_t$.  In NLG applications, we have $\mathcal{A} = \mathcal{V}$, where $\mathcal{V}$ is the vocabulary.  The transition function is deterministic and simply concatenates the present state with the chosen action to enter a new state.  Running the policy for $T$ time steps produces a fully generated sequence $\bhat y$.  

In order to train the policy, reinforcement learning requires the final component of the MDP -- a local loss (i.e. negative reward) function that evaluates the cost of the policy taking action $a$ in state $s$.  We would like the sum of this local reward function over the policy's visited states and selected actions to approximately yield a sequence-level metric that correlates with human judgement of generation quality.  However, many metrics for evaluating generation quality (e.g. BLEU score) cannot be easily decomposed into a simple sum over local rewards at the token level, which makes the local loss difficult to define in general. \hc{This is not entirely true. RL can be defined without intermediate rewards (assigning them to zero except for the end state). We can even assign BLEU-so-far as intermediate reward as a contrived example. The point we want to make is that we want to generate intermediate/granular rewards and we believe that it contains better information.}


% At test time, the autoregressive model is tasked with generating a full target sequence $\bhat{y}$ from scratch given a source feature $\bd x'$.  For example, in German-English translation, $\bd x'$ would be a German sentence and $\bhat{y}$ would be the model's decoded English sentence.   

% Generation is a sequential decision-making problem that can be cast in a reinforcement learning (RL) framework.  The Markov Decision Process (MDP) $(\mathcal{S}, \mathcal{A}, F, R)$ for generation can be defined as follows: The set of states $\mathcal{S}$ comprises all possible realizations of a partial target sequence given a source feature, i.e. all $s = \bd y_{<t} \given \bd x$.  Thus, each full target sequence $\bd y \given \bd x$ can be mapped to $T$ distinct states $\{\bd y_{<1}|\bd x, \ldots, \bd y_{<T}|\bd x\}$.  Each action $a \in \mathcal{A}$ is the next token in the target sequence, $a = y_t$, with the action set $\mathcal{A}$ being equal to the vocabulary $\mathcal{V}$ for natural language generation tasks.  The transition function $F : \mathcal{S} \times \mathcal{A} \to \mathcal{S}$ is deterministic and simply concatenates the present state with the chosen action to enter a new state $F(s, a) = F(\bd y_{<t} \given \bd x, {y}_t) = \bd y_{<t+1} \given \bd x$.  The ultimate goal of any generation problem is to learn a \emph{policy} $\pi : \mathcal{S} \to \mathbb{P}(\mathcal{A})$ that will walk along this MDP at test time to yield a fully generated sequence $\bhat y$.  

% In order to train the policy, we need the final component of the MDP -- a local reward function $R : \mathcal{S} \times \mathcal{A} \to [0, 1]$ that evaluates the benefit of the policy taking action $a$ in state $s$.  We would like the sum of this local reward function over the policy's visited states and selected actions to approximately yield a global, sequence-level metric $J(\pi)$ that correlates with human judgement of generation quality.  However, many metrics for evaluating generation quality (e.g. BLEU score) cannot be easily decomposed into a simple sum over local rewards at the token level, which makes $R$ difficult to define in general.

\subsection{Imitation Learning}

The field of \emph{imitation learning} (IL) tackles the problem of not having local supervision \hc{again this is not necessarily the motivation for IL. AFAIK, IL aims to learn from demonstration (e.g. state-action pairs) rather than reward.} by introducing an \emph{oracle} policy $\pi^*: \mathcal{S} \to \mathbb{P}(\mathcal{A})$ that is known to achieve high global score.  With such an oracle, we can recast the entire learning process as minimizing the divergence of the policy learner $\pi$ from the oracle $\pi^*$.  For example, it may be difficult to objectively define what it means for an aspiring translator to perform well (especially at the local word-by-word level).  Yet, if we were given access to an expert translator, we could simply say the learner is performing well if they translate in the same way as the expert. \hc{yes this is the motivation for IL and we can describe this property succinctly at the beginning}  Formally, IL trains the learner $\pi$ to minimize the local cost of its action being different from that of the oracle $\pi^*$ on a particular distribution (or dataset) $\mathcal{D}$ of states $\{s_1, \ldots, s_T\}$ visited by the $T$-step MDP:
\begin{align}
\mathcal{L}_{\text{imit}}(\pi) &= \E_{s_1, \ldots, s_T \sim \mathcal{D}}\left[\sum_{t=1}^T \ell^{\pi^*}(\pi, s_t)\right]. \label{imit}
\end{align}
Here, $\ell^{\pi^*}(s, \pi)$ is the oracle-dependent local loss functional of policy $\pi$ in state $s$.  A suitable candidate for this local loss is the negative log-likelihood of the optimal oracle action $a^* = \arg \max_a \pi^*(s)$,
\begin{align}
\ell^{\pi^*}_{\text{opt}}(\pi, s) = - \log \pi(a^* \given s). \label{nll-local}
\end{align}

% A sensible definition for this local loss is the disagreement probability between the oracle and the learner, $\ell^{\pi^*}_{\text{disagree}}(\pi, s) = 1 - \pi(a^* \given s)$, where $a^*$ is the optimal oracle action in state $s$. 

% , which upperbounds $\ell^{\pi^*}_{\text{disagree}}$ and is relevant in machine learning contexts,


In the setting of autoregressive distillation, the IL framework is quite attractive because the student naturally fills the role of the learner and the teacher naturally fills the role of the oracle.  This allows us to easily apply theoretical results and practical methods from the IL literature to better understand the autoregressive distillation problem.

\subsection{Teacher Forcing as Behavioral Cloning} \label{tf-as-bc}

One distinguishing feature between different imitation learning methods is how to define the distribution of states $\mathcal{D}$ in Equation \ref{imit}.  The simplest form of imitation learning is \emph{behavioral cloning} \citep{ross2010efficient}, which uses states $\mathcal{D}^*$ obtained by running the oracle $\pi^*$ on the MDP.

Teacher forcing training objectives for autoregressive models can be interpreted as special cases of behavioral cloning.  The vanilla objective with the original dataset (Equation \ref{nll}) can be seen as behavioral cloning with a human ``oracle", while seqKD (Equation \ref{seqkd}) is behavioral cloning with a teacher model as the ``oracle".  Indeed, we can show that the behavioral cloning objective (Equation \ref{imit}) with the optimal action local loss (Equation \ref{nll-local}) reduces to the following:  
\begin{align}
&\mathcal{L}_{\text{imitBC}}(\pi) = \E_{s_1, \ldots, s_T \sim \mathcal{D}^*}\left[\sum_{t=1}^T \ell^{\pi^*}_{\text{opt}}(\pi, s_t)\right] \\
&= \E_{\bd y^*|\bd x' \sim \mathcal{D}^*} \left[- \sum_{t=1}^T  \log  \pi(y_t^*\given \bd y_{<t}^*, \bd x')\right] \nonumber \\ 
&= \mathcal{L}_\text{seqKD}(\pi). \nonumber 
\end{align}

\citet{ross2010efficient} argued that training a policy $\pi$ via behavioral cloning incurs regret with respect to the oracle $\pi^*$ that is a quadratic function of the time horizon $T$.  %More specifically, they showed that if $\pi$ is a policy satisfying $\Loss_\text{imit-BC}(\pi) \leq \epsilon$,  then the student's global score is tightly bounded as follows: $J(\hat{\pi}) \geq J(\pi^*) - T^2 \epsilon$.  
Intuitively, the learner trained with behavioral cloning suffers from the \emph{exposure bias problem} \hc{We probably want to mention this in intro also}.  It is not exposed to its own distribution of states during training, so the errors compound during testing, when it can no longer apply teacher forcing. \hc{What do you mean by teacher forcing no longer applies?}

The key advantage of behavioral cloning lies in its simplicity; there may be many instances in which we do not have access to a dynamic oracle, but we do have some of its samples to work with.  One common example is a static machine translation dataset, which consists of a finite number of manually-translated sentences from a human ``oracle", but nothing more.  However, in the setting of autoregressive distillation, there does exist a teacher capable of correcting the student.  We argue that this is an ideal situation for employing more interactive imitation learning methods with the potential to ameliorate exposure bias. \hc{This paragraph could be a bit more concise.}

\subsection{Dataset Aggregation}

The dataset aggregation (DAgger) algorithm \citep{ross2011reduction} is one of the most popular imitation learning methods to improve upon behavioral cloning.  It is founded on the principle that at test time, the policy learner $\pi$ relies on its own state distribution for generation, so the learner should be trained on this same state distribution as well.  In practice, the states $s$ are typically sampled using an oracle-learner mixture policy $\tilde{\pi} = \beta \pi^* + (1 - \beta) \pi$, where $\beta \in [0, 1]$ is annealed during training.  This is done to alleviate the cold-start problem in the beginning of training, when the randomly initialized policy learner visits suboptimal states.      

% It works well in practice and is simple to implement.  Since its invention, it has also served as the basis for several other imitation learning algorithms \citep{he2012imitation, ross2014reinforcement, sun2017deeply}.



% This is because during the beginning of the training process, the learner is often randomly initialized and visits suboptimal states that are not useful for learning how to generate, so the oracle's states are also provided as a better starting point.  Given state $s \sim \mathcal{D}^{\tilde{\pi}}$, the correct action distribution is obtained by querying the oracle $\pi^*$ with state $s$; of course, this requires $\pi^*$ to be a dynamic entity capable of processing any potential state the learner could visit.  

DAgger works in a stepwise fashion, using the oracle to provide training signal to the learner $\pi$ over several iterations $i = 1, 2, \ldots, I$.  In each iteration $i$, we sample a new dataset $\mathcal{D}_i$ of states and train a new policy $\pi_{i}$ on an aggregated dataset $\mathcal{D}$ of the previous state distributions $\{\mathcal{D}_1, \ldots, \mathcal{D}_i\}$ by minimizing $\mathcal{L}_{\text{imit}}$ (Equation \ref{imit}).  The full DAgger algorithm is given in the appendix.

\algblockdefx{MRepeat}{EndRepeat}{\textbf{repeat} }{}
\algnotext{EndRepeat}

% \begin{algorithm}[H]
% \caption{Dataset Aggregation} \label{dagger}
% \begin{algorithmic}[1]
% \State Initialize dataset $\mathcal{D} = \emptyset$ and policy learner $\pi^1$ at random.
% \For {$i = 1, \ldots, I$}
%     \State Let mixture policy $\tilde{\pi}^i = \beta^i \pi^* + (1 - \beta^i) \pi^i$.
%     \State {Initialize new dataset $\mathcal{D}^i = \emptyset$.}
%     \MRepeat {$B$ \textbf{times}}
%         \State Run MDP on $\tilde{\pi}^i$, sample $\{s_1, \ldots, s_T\}$.
%         \State Append new states $\{s_1, \ldots, s_T\}$ to $\mathcal{D}^i$.
%     \EndRepeat
%     \State Aggregate $\mathcal{D} = \mathcal{D} \cup \mathcal{D}^i$.
%     \State Train $\pi^{i+1}$ on $\mathcal{D}$ to min $\Loss_{\text{imit}}$ with $\pi^*$.
% \EndFor \\
% \Return Best policy $\pi$ among $\pi^1, \ldots, \pi^I$ on validation set.
% \end{algorithmic}
% \end{algorithm}

Under some assumptions (the most significant of which requiring that the local loss $\ell^{\pi^*}$ be strongly convex in $\pi$), \citet{ross2011reduction} proved that DAgger yields a policy learner $\pi$ that has linear regret in $T$ with respect to $\pi^*$.  This is a significant improvement over the behavior cloning result and shows that DAgger can fix exposure bias by making the additional error constant at each time step.  The result is not guaranteed in general for non-convex loss functions (e.g. neural networks), but DAgger-inspired algorithms have still demonstrated empirical success in these regimes \citep[e.g.][]{zhang2016query, sun2017deeply}.


==> method.v2.tex <==
\section{Imitation-Based Distillation Algorithm}

We describe in this section our algorithm for autoregressive distillation.
Our algorithm builds upon the empirical and theoretical foundation of dataset aggregation (DAgger), one of the most popular imitation learning methods to improve upon behaviorial cloning.
We briefly introduce the original DAgger algorithm~\cite{ross2011reduction} and then describe our algorithm that is more amenable for training neural generative models.

\subsection{Dataset Aggregation}
The principle of DAgger and other related algorithms including ours is that the policy learner must be trained and be capable of relying on its own state distribution for generation.

Durining training, DAgger produces a state distribution $\mathcal{D}_{\tilde{\pi}}$ by sampling from an oracle-learner mixture 
$\tilde{\pi} = \beta \pi^* + (1 - \beta) \pi$, where $\beta \in [0, 1]$ is annealed during training. 
The annealing is used to alleviate the cold-start problem that the learner works poorly initially. 
DAgger trains $\pi$ over several iterations $i = 1, 2, \ldots, I$. 
In each iteration $i$, it generates a new dataset $\mathcal{D}_i$ (using current mixture $\tilde{\pi}_i$), and re-train the policy learner on an aggregated dataset consisting of $\mathcal{D}_i$ and all previous versions $\mathcal{D}=\{\mathcal{D}_1, \ldots, \mathcal{D}_i\}$.
%by minimizing $\mathcal{L}_{\text{imit}}$ (Equation \ref{imit}).
%\tl{The full DAgger algorithm is given in the appendix. (?)}

\algblockdefx{MRepeat}{EndRepeat}{\textbf{repeat} }{}
\algnotext{EndRepeat}

% \begin{algorithm}[H]
% \caption{Dataset Aggregation} \label{dagger}
% \begin{algorithmic}[1]
% \State Initialize dataset $\mathcal{D} = \emptyset$ and policy learner $\pi^1$ at random.
% \For {$i = 1, \ldots, I$}
%     \State Let mixture policy $\tilde{\pi}^i = \beta^i \pi^* + (1 - \beta^i) \pi^i$.
%     \State {Initialize new dataset $\mathcal{D}^i = \emptyset$.}
%     \MRepeat {$B$ \textbf{times}}
%         \State Run MDP on $\tilde{\pi}^i$, sample $\{s_1, \ldots, s_T\}$.
%         \State Append new states $\{s_1, \ldots, s_T\}$ to $\mathcal{D}^i$.
%     \EndRepeat
%     \State Aggregate $\mathcal{D} = \mathcal{D} \cup \mathcal{D}^i$.
%     \State Train $\pi^{i+1}$ on $\mathcal{D}$ to min $\Loss_{\text{imit}}$ with $\pi^*$.
% \EndFor \\
% \Return Best policy $\pi$ among $\pi^1, \ldots, \pi^I$ on validation set.
% \end{algorithmic}
% \end{algorithm}

Under some assumptions such as the loss function $\ell_\pi^{\pi^*}$ being strongly convex in $\pi$, \citet{ross2011reduction} proved that DAgger yields a policy learner $\pi$ that has linear regret in $T$ with respect to $\pi^*$.  
This is a significant improvement over the behavior cloning result by making the additional error constant at each time step.  
%Although the result is not guaranteed in general for non-convex loss functions (e.g. neural networks), 
Other DAgger-inspired algorithms have demonstrated empirical success for non-convex optimization (e.g. training neural networks) as well \citep[e.g.][]{zhang2016query, sun2017deeply}.

\subsection{Our Algorithm}
Our imitation learning based algorithm is given in Algorithm \ref{imit-alg}.  
We use the commonly adopted source-target $(\bd x, \bd y)$ notation in NLP instead of the state-action $(s, a)$ notation.
The central training objective of our algorithm is,
\begin{align}
\Loss_{\text{imitKD}}(\pi) = \E_{\bd y|\bd x \sim \tilde{\mathcal{D}}} \left[\sum_{t=1}^T \ell^{\pi^*}(\pi, \bd y_{<t} | \bd x) \right] \label{imitKD-loss}
\end{align}
where $\tilde{\mathcal{D}}$ is the data mixture defined by sampling from the initial dataset $\mathcal{D}$ or by performing the generation using the student (line 8-11).
%for some dataset $\mathcal{D}$. 
The loss function $\ell^{\pi^*}$ can be realized as the negative log-likelihood of the best token specified by the oracle
\begin{align}
\ell^{\pi^*}_{\text{opt}}(\pi, \bd y_{<t} \given \bd x) = - \log \pi(v^* \given \bd y_{<t}, \bd x), \nonumber
\end{align}
where $v^* = \arg \max_{v \in \mathcal{V}} \pi^*(v \given \bd y_{<t}, \bd x)$.
Alternatively, $\ell^{\pi^*}$ can be the cross-entropy loss between the full distributions,
\begin{align}
&\ell^{\pi^*}_{\text{full}}(\pi, \bd y_{<t} \given \bd x) \label{full} \nonumber\\
&= -\sum_{v \in \mathcal{V}} \pi^*(v \given \bd y_{<t}, \bd x) \cdot \log \pi(v \given \bd y_{<t}, \bd x). \nonumber
\end{align}
We next describe several practical design choices for distilling deep learning models.
%Our algorithm differs from the original DAgger algorithm in several aspects.

\begin{algorithm}[!th]
\caption{Imitation-Based Distillation} \label{imit-alg}
\begin{algorithmic}[1]
\State Let $\mathcal{D}$ be initial dataset.
\State Initialize $\pi_1$ at random.
\For {$i = 1, \ldots, I$}
    \State {Initialize new dataset $\tilde{\mathcal{D}}_i = \emptyset$.}
    \MRepeat {$B$ \textbf{times}}
        \State Sample an example $e = \bd y \given \bd x \sim \mathcal{D}$.
        \State Sample uniformly $u \sim [0, 1]$.
        \If {$u > \beta_i$} 
            \State Generate $\bhat{y}$ from $\pi_i$ given $\bd x$.
            \State Replace example with $e = \bhat y \given \bd x$.
        \EndIf
        \State Append example $e$ to $\tilde{\mathcal{D}}_i$.
    \EndRepeat
    \State Compute $\Loss_{\text{imitKD}}(\pi_i)$ on $\tilde{\mathcal{D}}_i$ with $\pi^*$.
    \State Let $\pi_{i+1} = \pi_i - \alpha_i \cdot \partial \Loss_{\text{imitKD}} / \partial \pi_i$.
\EndFor \\
\Return Best policy $\pi$ among $\pi_1, \ldots, \pi_I$ on validation set.
\end{algorithmic}
\end{algorithm}

% is "resampling" a better word for replacement?
\subsection{Substituting Samples for Mini-batch Gradient Decent}
One expensive aspect of DAgger is the fact that the dataset is repeatedly aggregated over each iteration, making each policy training phase successively more expensive.
This is especially true for modern datasets in domains such as translation, which can sometimes contain millions of training examples.
As an alternative, we choose to iteratively \emph{replace} the dataset instead of aggregating.

As shown in Algorithm~\ref{imit-alg}, we treat each mini-batch $\tilde{\mathcal{D}}_i$ as a new iteration of the dataset.
We perform a single step of stochastic gradient decent (SGD) on $\Loss_\text{imitKD}$ (Equation \ref{imitKD-loss}) with respect to the parameters of the previous model $\pi_i$ to yield $\pi_{i+1}$, by substituting examples in the current mini-batch.
The total number of iterations $I$ becomes the number of gradient steps (and mini-batches) used to train the neural network.

%Each iteration of the original DAgger algorithm involves training the policy learner to completion on the current dataset.  This can be very expensive if the learner is a neural network.  We substitute this line with a single gradient descent step on $\Loss_\text{imitKD}$ (Equation \ref{imitKD-loss}) with respect to the parameters of the previous policy $\pi_i$ to yield $\pi_{i+1}$.  Thus, the total number of iterations $I$ becomes the number of gradient steps to train the neural network.

These practical algorithmic changes are inspired by theory.
The dataset aggregation algorithm \citep{ross2011reduction} is able to achieve its regret bounds on strongly convex losses because it reduces to the Follow-the-Leader algorithm for online learning \citep{kakade2009complexity}.  Our training paradigm can be similarly interpreted as an online gradient descent algorithm, which has comparable guarantees for strongly convex losses \citep{hazan2007logarithmic} and even certain non-strongly convex losses \citep{garber2019logarithmic}.  Variants of this paradigm have also been employed in other deep learning work \citep{bengio2015scheduled, sun2017deeply}.

\subsection{Selecting the Data Mixture and Annealing}
Dataset replacement requires us to have an initial dataset or state distribution that can be potentially replaced at each step.  A natural candidate for this initial dataset is the original supervised training data (denoted as $\mathcal{D'})$, which can be interpreted as a collection of samples from a human oracle.
Alternatively, we can use the seqKD dataset $\mathcal{D}^*$ that is built with generations from the teacher.

If we take samples from $\mathcal{D}'$ or $\mathcal{D}^*$ and replace some of them with student-generated samples, we have effectively created a dataset mixture.  Unlike DAgger, this mixture occurs at the sequence level instead of the token/state level, but it is a teacher-student mixture nonetheless.
%The mixture serves the purpose of providing good training signal to the student while its state distribution is poor at the beginning of training.
An advantage of mixing teacher and student policies at the sequence level (instead of the token level) is that it obviates the need to sample from the teacher during training, which can be quite expensive (since the teacher is a large neural network).  
Instead, the teacher only needs to be used for computing the batched loss, which is comparatively much cheaper.

The exact mixing schedule $\beta_1, \ldots, \beta_I$ is a customizable feature of Algorithm \ref{imit-alg}.  Empirically, we have found an exponential decay to work well:
\begin{align}
\beta_i = r^{i / I},
\end{align}
where $r \in (0, 1]$ is the final mixing rate.

\subsection{Speeding Up the Training}
%As shown in previous works that perform generation during training, the generation step is often a major bottleneck.  
Generating sequences $\bhat y$ on the fly during training (line 9) is often a major bottleneck.
We speed up this step with two levels of parallelization.
First, the generation step (lines 5-12) can be executed in parallel for the entire batch.
Additionally, the generation step can also be parallelized \emph{across} different batches.
%Given parallel generation hyperparameter $M > 1$, 
Specifically, we generate a large pool of $B \cdot M$ examples in parallel only once every $M$ iterations, where $B$ is the batch size and $M$ is a hyperparameter.
%This reduces the number of iterations in which generation is executed to $I / M$.
One caveat of this modification is that at iteration $i$, the loss function may no longer be computed on examples generated by the most recent set of model parameters, but rather parameters from up to $M$ iterations prior.  Nonetheless, we have found that setting $M$ to a small integer (e.g. 2-8) can speed up training time without impacting final model performance.

We use a greedy decoding or top-$K$ sampling with small $K$ to produce samples $\bhat y$ (line 9) in our algorithm.
These two strategies are efficient to run, works similarly to the generation at inference time, and have empirically worked well in our experiments.
Of course, the generation strategy can be customized for different tasks.
%The exact generation algorithm to employ for producing samples $\bhat y$ (line 9) is customizable.  Empirically, we have found greedy decoding and top-$K$ sampling with small $K$ to work well, since these are a) efficient to run and b) similar to what is used for evaluation.

\subsection{Selecting Models for Teacher and Student}
Transformers often attain state-of-the-art performance for common NLG tasks (e.g. translation, summarization).  On the other hand, RNNs (without self attention) generate much faster at inference time.  Thus, from a practitioner's standpoint, it may be most desirable to compress a high-performing Transformer teacher into a speedy and lightweight RNN student.  
We consider distilling a teacher into either a small Transformer or RNN model in our experiments.

%Algorithm \ref{imit-alg} is especially suitable for this setting. 
%First of all, the Transformer architecture is designed to produce next-token predictions in parallel, which makes it an efficient teacher.  
%\tl{So does RNN as well. This is not a particular advantage of Transfomer.}
%Given any student-generated sequence $\bhat y$, which maps to $T$ states $\{\bhat y_{<1}, \ldots, \bhat y_{<T}\}$, the Transformer can retrieve its optimal actions for all $T$ states at once.  Secondly, RNNs perform generation and NLL training with the same computational complexity.  Thus, it is efficient to execute generation during training with an RNN student.   

